FedMedICL: Towards Holistic Evaluation of Distribution Shifts in Federated Medical Imaging

For medical imaging AI models to be clinically impactful, they must generalize. However, this goal is hindered by (i) diverse types of distribution shifts, such as temporal, demographic, and label shifts, and (ii) limited diversity in datasets that are siloed within single medical institutions. While these limitations have spurred interest in federated learning, current evaluation benchmarks fail to evaluate different shifts simultaneously. However, in real healthcare settings, multiple types of shifts co-exist, yet their impact on medical imaging performance remains unstudied. In response, we introduce FedMedICL, a unified framework and benchmark to holistically evaluate federated medical imaging challenges, simultaneously capturing label, demographic, and temporal distribution shifts. We comprehensively evaluate several popular methods on six diverse medical imaging datasets (totaling 550 GPU hours). Furthermore, we use FedMedICL to simulate COVID-19 propagation across hospitals and evaluate whether methods can adapt to pandemic changes in disease prevalence. We find that a simple batch balancing technique surpasses advanced methods in average performance across FedMedICL experiments. This finding questions the applicability of results from previous, narrow benchmarks in real-world medical settings.

==> LatexSource/sections/7_acknowledgements.tex <==
\begin{credits}
\subsubsection{\ackname}
The authors thank Haoran Zhang for his feedback. Kumail was supported by a Jameel Clinic Fellowship and a Saudi Arabian Cultural Mission Scholarship. Yasir was supported by Saudi Aramco. Marzyeh is supported in part by an NSF CAREER award, a CIFAR AI Chair held at the Vector Institute, and the Gordon and Betty Moore Foundation. This project was also supported by the KAUST Office of Sponsored Research (OSR) under Award No. OSR-CRG2021-4648 and a UKRI grant Turing AI Fellowship (EP/W002981/1). Philip thanks the Royal Academy of Engineering for their support.

\subsubsection{\discintname}
The authors have no competing interests to declare that are relevant to the content of this article.
\end{credits}

==> LatexSource/tables/novel_and_foundation.tex <==
\begin{figure}[t]
\centering
\captionof{table}{\textbf{Novel Disease Detection.} We compare accuracy on common and novel diseases before and after the introduction of COVID-19. \textcolor{red}{WILL CHANGE}
}
\label{tab:novel_disease}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
& \multicolumn{2}{c}{\textbf{Pre-COVID}} & \multicolumn{2}{c}{\textbf{Post-COVID}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Model}  & \textbf{Common} & \textbf{Novel} & \textbf{Common} & \textbf{Novel} \\
               & \textbf{Acc.} & \textbf{Acc.} & \textbf{Acc.} & \textbf{Acc.} \\
\midrule
ERM           & 51.0$_{\pm 1.9}$ & 0.0 & 51.5$_{\pm 1.0}$ & 34.7$_{\pm 42.6}$ \\
FedAvg        & 58.6 & 0.0 & 56.7 & 83.3 \\
F-CB            & 63.1 & 0.0 & \textbf{62.7} & \textbf{88.9} \\
F-GB    & 59.1 & 0.0 & 57.7 & 77.8 \\
FACTR         & 63.1 & 0.0 & 60.8 & 66.7 \\
\bottomrule
\end{tabular}%
}
\end{figure}

